Learning Time/Memory-Efficient Deep Architectures with Budgeted Super Networks

We propose to focus on the problem of discovering neural network architectures efficient in terms of both prediction quality and cost. For instance, our approach is able to solve the following tasks: learn a neural network able to predict well in less than 100 milliseconds or learn an efficient model that fits in a 50 Mb memory. Our contribution is a novel family of models called Budgeted Super Networks (BSN). They are learned using gradient descent techniques applied on a budgeted learning objective function which integrates a maximum authorized cost, while making no assumption on the nature of this cost. We present a set of experiments on computer vision problems and analyze the ability of our technique to deal with three different costs: the computation cost, the memory consumption cost and a distributed computation cost. We particularly show that our model can discover neural network architectures that have a better accuracy than the ResNet and Convolutional Neural Fabrics architectures on CIFAR-10 and CIFAR-100, at a lower cost.

==> results/cifar100_resnetfab_para1.tex <==
\begin{table}[h]
\centering
\caption{Accuracy at different levels of parallelization (p=1) on Cifar-100 using ResNet Fabrics.}
\label{cif100_resnetfab_para1}
\begin{tabular}{|lll|}
\hline
Model        & \# of sequential operations & Accuracy (\%) \\ \hline \hline
ResNet110    & 112.00                      & 71.85         \\
ResNet56     & 58.00                       & 70.57         \\
ResNet44     & 46.00                       & 70.28         \\
ResNet32     & 34.00                       & 69.28         \\
ResNet20     & 22.00                       & 67.14         \\ \hline
ResNetFabric & 184.00                      & 73.85         \\
ResNetFabric & 110.00                      & 72.88         \\
ResNetFabric & 67.00                       & 72.02         \\
ResNetFabric & 32.00                       & 69.60         \\
ResNetFabric & 20.00                       & 68.48         \\ \hline
\end{tabular}
\caption{Accuracy at different levels of parallelization (p=1) on Cifar-100 using ResNet Fabrics.}
\label{cif100_resnetfab_para1}
\end{table}

==> results/cifar10_allmodels_allpara.tex <==
\begin{table}[]
\centering
\begin{tabular}{|lll|}
\hline
Model                       & \# of sequential operations & Accuracy \% \\ \hline \hline
PARA 1                      &                             &             \\ \hline 
ResNet-110                  & 112.00                      & 94.09       \\
ResNet-56                   & 58.00                       & 93.61       \\
ResNet-44                   & 46.00                       & 93.21       \\
ResNet-32                   & 34.00                       & 92.91       \\
ResNet-20                   & 22.00                       & 92.19       \\ \hline
ResNet-110 \cite{DBLP:journals/corr/HeZRS15}      & 110.00                      & 93.57       \\
ResNet-56 \cite{DBLP:journals/corr/HeZRS15}       & 56.00                       & 93.03       \\
ResNet-44 \cite{DBLP:journals/corr/HeZRS15}      & 44.00                       & 92.83       \\
ResNet-32 \cite{DBLP:journals/corr/HeZRS15}      & 32.00                       & 92.49       \\
ResNet-20 \cite{DBLP:journals/corr/HeZRS15}      & 20.00                       & 91.25       \\ \hline
B-ResNet                    & 184.00                      & 94.42       \\
B-ResNet                    & 110.00                      & 94.12       \\
B-ResNet                    & 94.00                       & 94.01       \\
B-ResNet                    & 22.00                       & 93.06       \\
B-ResNet                    & 20.00                       & 92.29       \\ \hline
CNF W=8                     & 171.00                      & 94.83       \\
CNF W=4                     & 83.00                       & 93.75       \\
CNF W=2                     & 39.00                       & 92.54       \\
CNF W=1                     & 12.00                       & 89.91       \\ \hline
CNF W=8 (Saxena \& Verbeek) & 171.00                      & 90.58       \\
CNF W=4 (Saxena \& Verbeek) & 83.00                       & 87.91       \\
CNF W=2 (Saxena \& Verbeek) & 39.00                       & 86.21       \\ \hline
Random CNF                  & 134.00                      & 93.99       \\
Random CNF                  & 21.00                       & 92.56       \\
Random CNF                  & 18.00                       & 88.64       \\ \hline
B-CNF                       & 98.00                       & 95.02       \\
B-CNF                       & 50.00                       & 94.62       \\
B-CNF                       & 45.00                       & 94.55       \\
B-CNF                       & 39.00                       & 94.35       \\
B-CNF                       & 33.00                       & 93.00       \\
B-CNF                       & 26.00                       & 92.91       \\
B-CNF                       & 18.00                       & 92.87       \\ \hline \hline
PARA 2                      &                             &             \\ \hline
ResNet-110                  & 110.00                      & 94.09       \\
ResNet-56                   & 56.00                       & 93.61       \\
ResNet-44                   & 44.00                       & 93.21       \\
ResNet-32                   & 32.00                       & 92.91       \\
ResNet-20                   & 20.00                       & 92.19       \\ \hline
ResNet-110 (He et al.)      & 110.00                      & 93.57       \\
ResNet-56 (He et al.)       & 56.00                       & 93.03       \\
ResNet-44 (He et al.)       & 44.00                       & 92.83       \\
ResNet-32 (He et al.)       & 32.00                       & 92.49       \\
ResNet-20 (He et al.)       & 20.00                       & 91.25       \\ \hline
B-ResNet                    & 179.00                      & 94.36       \\
B-ResNet                    & 112.00                      & 94.42       \\
B-ResNet                    & 56.00                       & 94.31       \\
B-ResNet                    & 20.00                       & 93.20       \\
B-ResNet                    & 18.00                       & 92.81       \\ \hline
CNF W=8                     & 90.00                       & 94.83       \\
CNF W=4                     & 47.00                       & 93.75       \\
CNF W=2                     & 26.00                       & 92.54       \\
CNF W=1                     & 12.00                       & 89.91       \\ \hline
CNF W=8 (Saxena \& Verbeek) & 90.00                       & 90.58       \\
CNF W=4 (Saxena \& Verbeek) & 47.00                       & 87.91       \\
CNF W=2 (Saxena \& Verbeek) & 26.00                       & 86.21       \\ \hline
Random CNF                  & 71.00                       & 93.99       \\
Random CNF                  & 18.00                       & 92.56       \\ \hline
B-CNF                       & 47.00                       & 94.67       \\
B-CNF                       & 30.00                       & 94.68       \\
B-CNF                       & 28.00                       & 94.58       \\
B-CNF                       & 24.00                       & 94.41       \\
B-CNF                       & 20.00                       & 94.35       \\
B-CNF                       & 18.00                       & 92.86       \\ \hline \hline
PARA 4                      &                             &             \\ \hline
ResNet-110                  & 110.00                      & 94.09       \\
ResNet-56                   & 56.00                       & 93.61       \\
ResNet-44                   & 44.00                       & 93.21       \\
ResNet-32                   & 32.00                       & 92.91       \\
ResNet-20                   & 20.00                       & 92.19       \\ \hline
ResNet-110 (He et al.)      & 110.00                      & 93.57       \\
ResNet-56 (He et al.)       & 56.00                       & 93.03       \\
ResNet-44 (He et al.)       & 44.00                       & 92.83       \\
ResNet-32 (He et al.)       & 32.00                       & 92.49       \\
ResNet-20 (He et al.)       & 20.00                       & 91.25       \\ \hline
B-ResNet                    & 110.00                      & 94.36       \\
B-ResNet                    & 58.00                       & 94.01       \\
B-ResNet                    & 20.00                       & 93.24       \\
B-ResNet                    & 18.00                       & 92.93       \\
B-ResNet                    & 16.00                       & 92.75       \\ \hline
CNF W=8                     & 53.00                       & 94.83       \\
CNF W=4                     & 31.00                       & 93.75       \\
CNF W=2                     & 19.00                       & 92.54       \\
CNF W=1                     & 12.00                       & 89.91       \\ \hline
CNF W=8 (Saxena \& Verbeek) & 53.00                       & 90.58       \\
CNF W=4 (Saxena \& Verbeek) & 31.00                       & 87.91       \\
CNF W=2 (Saxena \& Verbeek) & 19.00                       & 86.21       \\ \hline
Random CNF                  & 42.00                       & 93.99       \\
Random CNF                  & 18.00                       & 92.56       \\ \hline
B-CNF                       & 31.00                       & 94.96       \\
B-CNF                       & 25.00                       & 94.72       \\
B-CNF                       & 21.00                       & 94.36       \\
B-CNF                       & 18.00                       & 93.86       \\ \hline
\end{tabular}
\caption{Results for \textit{Distributed computation cost} on CIFAR-10}
\label{cif10_allpara}
\end{table}

==> results/cifar10_cnf_flops_mem.tex <==
\begin{table}[]
\centering
\caption{Accuracy/speed and accuracy/memory trade-offs on Cifar-10 using CNF.}
\label{cif10_cnf_flop_mem}
\begin{tabular}{|llll|}
\hline
Model                       & FLOPs $\times 1^8$ & \# params $\times 1^6$ & Accuracy (\%) \\ \hline \hline
CNF L=8                     & 22.19                 & 18.04                & 94.83         \\
CNF L=4                     & 10.10                 & 8.58                 & 93.75         \\
CNF L=2                     & 4.06                  & 3.85                 & 92.54         \\
CNF L=1                     & 0.54                  & 0.74                 & 89.91         \\ \hline
CNF L=8 \cite{DBLP:journals/corr/SaxenaV16} & 22.19                 & 21.00                & 90.58         \\
CNF L=4 \cite{DBLP:journals/corr/SaxenaV16} & 10.10                 & 10.00                & 87.91         \\
CNF L=2 \cite{DBLP:journals/corr/SaxenaV16} & 4.06                  & 5.00                 & 86.21         \\ \hline
Random CNF                  & 14.53                 & 13.61                & 93.99         \\
Random CNF                  & 1.58                  & 1.48                 & 92.56         \\
Random CNF                  & 0.57                  & 1.18                 & 88.64         \\ \hline
BSN                         & 21.50                 &                      & 94.92         \\
BSN                         & 14.07                 &                      & 94.85         \\
BSN                         & 11.44                 &                      & 94.69         \\
BSN                         & 1.03                  &                      & 93.14         \\
BSN                         & 0.85                  &                      & 92.17         \\ \hline
BSN                         &                       & 7.56                 & 94.88         \\
BSN                         &                       & 4.98                 & 94.58         \\
BSN                         &                       & 4.28                 & 94.55         \\
BSN                         &                       & 3.67                 & 94.42         \\
BSN                         &                       & 2.65                 & 94.00         \\
BSN                         &                       & 1.19                 & 93.53         \\ \hline
\end{tabular}
\caption{Accuracy/speed and accuracy/memory trade-offs on Cifar-10 using CNF.}
\label{cif10_cnf_flop_mem}
\end{table}

==> results/cifar10_resnetfab_flops.tex <==
\begin{table}[]
\centering
\caption{Accuracy/speed trade-off on Cifar-10 using ResNet Fabrics.}
\label{cif10_rnf_flop}
\begin{tabular}{|lll|}
\hline
Model                  & FLOPs (millions) & Accuracy \\ \hline
ResNet-110             & 253.7            & 94.09    \\
ResNet-56              & 126.01           & 93.61    \\
ResNet-44              & 97.64            & 93.21    \\
ResNet-32              & 69.27            & 92.91    \\
ResNet-20              & 40.9             & 92.19    \\ \hline
ResNet-110 (He et al.) & 253.7            & 93.57    \\
ResNet-56  (He et al.) & 126.01           & 93.03    \\
ResNet-44  (He et al.) & 97.64            & 92.83    \\
ResNet-32 (He et al.)  & 69.27            & 92.49    \\
ResNet-20 (He et al.)  & 40.9             & 91.25    \\ \hline
LCCL (ResNet-20)       & 26               & 91.68    \\
LCCL (ResNet-32)       & 49               & 92.56    \\
LCCL (ResNet-44)       & 65               & 92.71    \\ \hline
MSDNet (Huang et al.)  & 255              & 94.1     \\
MSDNet (Huang et al.)  & 225              & 94       \\
MSDNet (Huang et al.)  & 205              & 94       \\
MSDNet (Huang et al.)  & 180              & 94       \\
MSDNet (Huang et al.)  & 145              & 93.8     \\
MSDNet (Huang et al.)  & 119              & 93.7     \\
MSDNet (Huang et al.)  & 97               & 93.3     \\
MSDNet (Huang et al.)  & 80               & 92.8     \\
MSDNet (Huang et al.)  & 45               & 91.8     \\
MSDNet (Huang et al.)  & 25               & 90       \\ \hline
ResNetFabric           & 407.51           & 94.29    \\
ResNetFabric           & 152.6            & 94.01    \\
ResNetFabric           & 120.2            & 93.71    \\
ResNetFabric           & 56.47            & 92.92    \\
ResNetFabric           & 42.69            & 92.48    \\
ResNetFabric           & 39.25            & 92.39    \\ \hline
\end{tabular}
\caption{Accuracy/speed trade-off on Cifar-10 using ResNet Fabrics.}
\label{cif10_rnf_flop}
\end{table}


==> results/cifar10_resnetfab_param.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|}
\hline
Model               & \# params (millions) & Error(\%) \\ \hline
ResNet110           & 1.73                 & 5.91      \\
ResNet56            & 0.86                 & 6.39      \\
ResNet44            & 0.66                 & 6.79      \\
ResNet32            & 0.47                 & 7.09      \\
ResNet20            & 0.27                 & 7.81      \\ \hline
ResNet110 \cite{DBLP:journals/corr/HeZRS15} & 1.70                 & 6.43      \\
ResNet56  \cite{DBLP:journals/corr/HeZRS15} & 0.85                 & 6.97      \\
ResNet44  \cite{DBLP:journals/corr/HeZRS15} & 0.66                 & 7.17      \\
ResNet32 \cite{DBLP:journals/corr/HeZRS15}  & 0.46                 & 7.51      \\
ResNet20 \cite{DBLP:journals/corr/HeZRS15}  & 0.27                 & 8.75      \\ \hline
ResNetFabric        & 4.38                 & 5.65      \\
ResNetFabric        & 2.27                 & 5.80      \\
ResNetFabric        & 1.29                 & 6.15      \\
ResNetFabric        & 0.48                 & 6.58      \\
ResNetFabric        & 0.34                 & 7.28      \\
ResNetFabric        & 0.30                 & 7.48      \\
ResNetFabric        & 0.29                 & 7.83      \\ \hline
\end{tabular}
\caption{Accuracy/Memory Trade-off on Cifar 10 using ResNet Fabric}
\label{cif10_mem_rnf_tab}
\end{table}
